GPT-4 Jailbreaks Itself with Near-Perfect Success Using Self-Explanation

Research on jailbreaking has been valuable for testing and understanding the safety and security issues of large language models (LLMs). In this paper, we introduce Iterative Refinement Induced Self-Jailbreak (IRIS), a novel approach that leverages the reflective capabilities of LLMs for jailbreaking with only black-box access. Unlike previous methods, IRIS simplifies the jailbreaking process by using a single model as both the attacker and target. This method first iteratively refines adversarial prompts through self-explanation, which is crucial for ensuring that even well-aligned LLMs obey adversarial instructions. IRIS then rates and enhances the output given the refined prompt to increase its harmfulness. We find that IRIS achieves jailbreak success rates of 98% on GPT-4, 92% on GPT-4 Turbo, and 94% on Llama-3.1-70B in under 7 queries. It significantly outperforms prior approaches in automatic, black-box, and interpretable jailbreaking, while requiring substantially fewer queries, thereby establishing a new standard for interpretable jailbreaking methods.

==> sections/related_works.tex <==
As LLM proficiency has increased, so too has the breadth of jailbreak research, leading to a more well-defined variety of automatic approaches. Distinctions between types of jailbreaks include their associated "failure modes", which identify two methods under which an LLM responds to an attack: "competing objectives", which exploits LLMs' instruction-following objective, and "mismatched generalization", which exploits LLM knowledge beyond its safety guardrails \cite{wei2024jailbroken}. Jailbreaks can be categorized as either "prompt-level" or "token-level" to describe the type of edits made to an initial adversarial prompt in order to produce a jailbreak \cite{chao2023jailbreaking}. Furthermore, there is a distinction between jailbreaks that use black-box access and white-box access to LLMs, and those that involve fine-tuning LLMs to generate jailbreak prompts. 

White-box access to the weights of LLMs such as Vicuna-7B and Llama-2-7B-Chat enable gradient-based jailbreaks by optimizing an adversarial suffix to a harmful prompt \cite{zou2023universal}. Gradient-based methods often produce uninterpretable prompts that can be defended using perplexity filters \cite{alon2023detecting}. Optimizing tokens one at a time in order promotes readability for gradient-based adversarial suffixes that can bypass perplexity filters \cite{zhu2023autodan}. However, white-box approaches cannot be used directly on GPT models without open access to model weights, and transferring prompts optimized on open-source LLMs is suboptimal. This suggests that not only is interpretability is an important factor when producing jailbreak prompts, but also that white-box jailbreaking methods do not provide reproducible jailbreaks on more advanced black-box LLMs. 

%\citet{zou2023universal} presents Greedy Coordinate Gradient (GCG), which uses white-box access to Vicuna-7B and Llama-2-7B-Chat to optimize an adversarial suffix to a harmful prompt. GCG achieves 99\% jailbreak success on Vicuna-7B and 56\% success on Llama-2, however, it cannot be used directly on GPT models without access to model weights. When using prompts optimized by GCG on Vicuna and Guanacos, at least one of the prompts jailbreaks GPT-4 only 47\% of the time. This method demonstrates the efficacy of white-box jailbreaks on models with open access to model weights, but it produces prompts that are uninterpretable and unable to be directly applied to more advanced LLMs that only provide black-box access. Since uninterpretable prompts can be defended using perplexity filters \cite{alon2023detecting}, AutoDAN \cite{zhu2023autodan} provides an  improvement on GCG by producing interpretable prompts with gradient-based adversarial suffixes. AutoDAN achieves 88\% jailbreak success on Vicuna with a perplexity filter, while GCG only achieves 21\%. This suggests that interpretability is an important factor when producing jailbreak prompts. However, AutoDAN still is not effective on GPT-4, achieving only a 29\% jailbreak success rate. These results suggest that white-box jailbreaking methods do not provide reproducible jailbreaks on more advanced LLMs. 

An alternative to white-box optimization is fine-tuning a an LLM to generate modified prompts using various persuasion techniques \cite{zeng2024johnny}. Since advanced LLMs reject requests to modify harmful requests, 
fine-tuning GPT-3.5 to bypass this restriction can succesfully generate a set of adversarial prompts using each persuasion technique. Aside from the resources needed to train the paraphraser, testing each prompt in the set requires many queries to successfully jailbreak GPT-4. 

%An alternative to white-box optimization is fine-tuning a an LLM to generate modified prompts, as done in \citet{zeng2024johnny} with Persuasive Adversarial Prompts (PAP). Since advanced LLMs reject requests to modify harmful requests, \citet{zeng2024johnny} fine-tunes GPT-3.5 to modify harmful prompts using various persuasion techniques. Across 400 attempts, PAP successfully achieves at least one jailbreak 92\% of the time on GPT-4 when evaluated using GPT-4. However, this success decreases to 72\% when each of the 40 persuasion techniques is only attempted once.

For larger LLMs with only black-box access, methods leveraging the more advanced capabilities of these models to jailbreak them become feasible. Many-shot jailbreaking uses in-context learning within a single prompt to fake an agreeable dialogue between the AI assistant and a harmful agent, before ultimately including the target adversarial prompt at the end \cite{anilmany}. Other black-box methods use smaller models like Vicuna-13B to iteratively refine an input prompt until the target LLM produces a response. Variants include PAIR \cite{chao2023jailbreaking} and TAP \cite{mehrotra2023tree}, which use chain-of-thought and tree-of-thought reasoning, respectively, to generate prompt modifications of the AdvBench Subset dataset. The tree-of-thought approach can require more complex methods like pruning off-topic prompts, but ultimately provides better results , although both methods require many iterations before successfully jailbreaking. Our work builds on the results of these black-box approaches, using GPT-4 and GPT-4 Turbo as our target LLMs for jailbreaking due to their popularity and strong alignment, while leveraging their inherent capabilities to induce jailbreaks.

%Our work builds on the results of \citet{chao2023jailbreaking, mehrotra2023tree}, using GPT-4 and GPT-4 Turbo as our target LLMs for jailbreaking due to their popularity and strong alignment. \citet{chao2023jailbreaking} proposes PAIR, in which Vicuna-13B-v1.5 is used to iteratively refine an input prompt until the target LLM produces a response. They use the AdvBench Subset dataset of 50 harmful prompts, on which PAIR achieves a 62\% success rate with an average of 16.6 queries. \citet{mehrotra2023tree} presents TAP, which uses tree-of-thought reasoning to generate prompt modifications of the AdvBench Subset dataset with more diversity and prunes off-topic prompts until a jailbreak is reached. They determine when a response is a jailbreak using GPT-4 as an evaluator, for which TAP achieves a 90\% success rate on GPT-4 as a target with an average of 28.8 queries and an 84\% success rate on GPT-4 Turbo with an average of 22.5 queries. When evaluating the jailbreaks using human judgment, however, GPT-4 is jailbroken with a success rate of 74\% and GPT-4 Turbo with a rate of 76\%. We follow the frameworks of PAIR and TAP, evaluating on the AdvBench Subset dataset and measuring the number of queries required to successfully jailbreak the target LLM. We will compare our results to the human evaluation metrics, since GPT-4 evaluation proves to be erroneous (Figure \ref{fig:diagram}).
